Constraints on cosmic strings using data from the first Advanced LIGO observing run

Cosmic strings are topological defects which can be formed in GUT-scale phase transitions in the early universe. They are also predicted to form in the context of string theory. The main mechanism for a network of Nambu-Goto cosmic strings to lose energy is through the production of loops and the subsequent emission of gravitational waves, thus offering an experimental signature for the existence of cosmic strings. Here we report on the analysis conducted to specifically search for gravitational-wave bursts from cosmic string loops in the data of Advanced LIGO 2015-2016 observing run (O1). No evidence of such signals was found in the data, and as a result we set upper limits on the cosmic string parameters for three recent loop distribution models. In this paper, we initially derive constraints on the string tension $G\mu$ and the intercommutation probability, using not only the burst analysis performed on the O1 data set, but also results from the previously published LIGO stochastic O1 analysis, pulsar timing arrays, cosmic microwave background and Big-Bang nucleosynthesis experiments. We show that these data sets are complementary in that they probe gravitational waves produced by cosmic string loops during very different epochs. Finally, we show that the data sets exclude large parts of the parameter space of the three loop distribution models we consider.

==> data_red.tex <==
\section{Constraining cosmic strings models with GW data}\label{sec:data}

\subsection{Gravitational waves from cosmic strings}\label{sec:data:gw}

GW bursts are emitted by both cusps and kinks on cosmic string loops, the frequency-domain waveform of which was calculated in~\cite{Damour:2000wa,Damour:2001bk,Damour:2004kw}:
\be
h(\ell,z,f) = A_q(\ell,z) f^{-q} \Theta(f_h-f)\Theta(f-f_\ell),
\label{eq:wf}
\ee
where $q=4/3$ for cusps, $q=5/3$ for kinks, and $A_q(\ell,z)$ is the signal amplitude produced by a cusp/kink propagating on a loop of size $\ell$ at redshift $z$. This waveform is linearily polarized and is only valid if the beaming angle 
\be
\theta_m(\ell,z,f) \equiv (g_2 f (1+z)\ell)^{-1/3} < 1.
\label{thetam}
\ee
Here $g_2$ is an ignorance factor assumed to be 1 in this work (see~\cite{Siemens:2006vk}). In order to detect the GW, the angle subtended by the line of sight and the cusp/kink on a loop of typical invariant length $\ell$ at redshift $z$, must be smaller than $\theta_m$. This condition then determines the high-frequency cutoff $f_h$ in Eq.~\ref{eq:wf}. The low-frequency cutoff $f_\ell$ --- though in principle determined by the kink amplitude, or by the size of the feature that produces the cusp --- is in practice given by the lower end of the GW detector's sensitive band. The amplitude $A_q(\ell,z)$ is given by~\cite{Damour:2001bk}
\be
A_q(\ell,z) = g_1 \frac{G\mu \ell^{2-q}}{(1+z)^{q-1}r(z)}~,
\label{eq:A}
\ee
where the proper distance to the source is given by $r(z) = H_{0}^{-1} \varphi_r(z)$. Here, $H_0$ is the Hubble parameter today and $\varphi_r(z)$ is determined in terms of the cosmological parameters and expressed in Appx.~\ref{appx:cosmo}. Finally $g_1$ gathers together a certain number of uncertainties which enter into the calculation of the cusp and kink waveform (including the amplitude of the cusp/kink, as well as numerical factors of order 1, see~\cite{Damour:2001bk,Siemens:2006vk}). We will set $g_1=1$. In the following, we will use Eq.~\ref{eq:A} to conveniently choose 2 variables out of $\ell$, $z$ and $A_q$. Similarly, we will use Eq.~\ref{eq:wf} to substitute $A_q$ for the strain amplitude $h$.

For a given loop distribution model $M$, in the following we use the GW burst rate derived in~\cite{Siemens:2006vk} and recalled in Appx.~\ref{appx:tech}:
\ba
\frac{d^2R^{(M)}_{q}}{dzdh}(h,z,f) &=& \frac{2N_qH_0^{-3}\varphi_V(z)}{(2-q)(1+z)ht^4(z)} \nonumber \\
&& \times {\cal F}^{(M)}\left(\frac{\ell(hf^q,z)}{t(z)},t(z)\right)  \nonumber \\
&& \times \Delta_{q}(hf^q,z,f).
\label{eq:d2Rdzdh}
\ea
The first two lines on the right-hand side give the number of cusp/kink features per unit space-time volume on loops of size $\ell$, where $N_{q}$ is the number of cusps/kinks per oscillation period $T=\ell/2$ of the loop. In this paper, the number of cusps/kinks per loop oscillation is set to 1 although some models~\cite{Binetruy:2010cc} suggest that this number can be much larger than one. Cosmic time is given by $t(z)=\varphi_t(z)/H_0$ and the proper volume element is $dV(z) = H_0^{-3} \varphi_V(z) dz$ where $\varphi_t(z)$ and $\varphi_V(z)$ are given in Appx.~\ref{appx:cosmo}. Finally $\Delta_q$, which is fully derived in Appx.\ref{appx:tech}, is the fraction of GW events of amplitude $A_q$ that are observable at frequency $f$ and redshift $z$.

\subsection{Gravitational-wave bursts}\label{sec:data:bursts}
We searched the
Advanced LIGO O1 data (2015-2016)~\cite{TheLIGOScientific:2016agk} for individual bursts of GWs from cusps and
kinks. The search for cusp signals was previously conducted using initial LIGO and Virgo data and no signal was found~\cite{Aasi:2013vna}.

For this paper, we use the same analysis pipeline to search for both cusp and kink signals. We perform a Wiener-filter analysis to identify events matching the waveform predicted by the theory~\cite{Damour:2000wa,Damour:2001bk,Damour:2004kw} and given in Eq.~\ref{eq:wf}. GW events are detected by matching the data to a bank of waveforms parameterized by the high-frequency cutoff $f_h$, with $30$~Hz~$<f_h<4096$~Hz. Then resulting events detected at LIGO-Hanford and at LIGO-Livingston are set in time coincidence to reject detector noise artifacts mimicking cosmic string signals. Finally, a multivariate likelihood ratio~\cite{Cannon:2008zz} is computed to rank coincident events and infer probability to be signal or noise. The analysis method is described in~\cite{Aasi:2013vna}. In this paper we only report on the results obtained from the analysis of new O1 LIGO data.

The upper plots in Fig.~\ref{fig:burst} present the final event rate as a function of the likelihood ratio $\Lambda$ for the cusp and kink search. The rate of accidental coincident events between the two detectors (background) is estimated by performing the analysis over 6000 time-shifted LIGO-Livingston data sets. This background data set virtually offers $2.5 \times 10^{10}$~s ($\sim 790.7$~years) of double-coincidence time.  For both cusps and kinks, the candidate ranking values are compatible with the expected background distribution, so no signal was found. The highest-ranked event is measured with $\Lambda_h \simeq 232$ for cusps and $\Lambda_h \simeq 611$ for kinks. These events were scrutinized and were found to belong to a known category of noise transients called ``blips'' described in~\cite{TheLIGOScientific:2016zmo}, matching very well the waveform of cusp and kink signals. 

The sensitivity to cusp and kink GW events is estimated experimentally by injecting simulated signals of known amplitude $A_q$ in the data. We measure the detection efficiency $e_q(A_q)$ as the fraction of simulated signals recovered with $\Lambda > \Lambda_h$, which is associated to a false alarm rate of $1/T_{\rm{obs}}=2.40\times 10^{-7}$~Hz. The detection efficiencies are displayed in the bottom plots in Fig.~\ref{fig:burst}. The sensitivity curve of the 2005-2010 LIGO-Virgo cusp search is also plotted, and should be compared with the O1 LIGO sensitivity measured for an equivalent false-alarm rate of $1.85 \times 10^{-8}$~Hz~\cite{Aasi:2013vna}. The sensitivity to cosmic string signals is improved by a factor 10. This gain is explained by the significant sensitivity improvement at low frequencies of Advanced detectors~\cite{TheLIGOScientific:2016agk}.

%In order to understand what one could learn from a burst-type detection, let us assume one signal was detected in the observation time $T_{\rm{obs}}$ and let us use Fig.~\ref{fig:rate1}. At $f=100$~Hz, ground-based GW detectors are typically sensitive to strain amplitudes of $h\sim10^{-23}$. Fixing the string tension $G\mu$ at $10^{-8}$, we see that the experimental observation time is compatible with the GW rate predicted by model 3, while for models 1 and 2 it is less compatible. Moreover, the detected signal would be most likely attributed to a cusp propagating on a string loop originally produced with a large size in the radiation era ($\alpha > \Gamma G\mu$). The loop size decreased over time until some point in the matter era when the GW burst was produced. Indeed, we know that the detection probability increases for smaller loops due to larger beaming angles. This effect explains why the chance of detection is higher for a signal emitted in the matter era.

Since no signal from cosmic string was found in LIGO O1 data, it is possible to constrain cosmic string parameters using models 1, 2 and 3. To generate statistical statements about our ability to detect true GW signals, we adopt the loudest event statistic~\cite{Brady:2004gt}. We compute an effective detection rate for a given loop distribution model $M$ :
\ba
   {\cal{R}}^{(M)}_q(G\mu,p) &=& \int_0^{+\infty}dA_q\ e_q(A_q) \\
     && \times \int_0^{+\infty}{dz\frac{d^2R^{(M)}_q}{dzdA_q}(A_q,z,f^{*};G\mu,p)},
\label{eq:R}
\ea
where the predicted rate is given by Eq.~\ref{eq:d2Rdzdh} with the change of variables $A_q=hf^{-q}$. The frequency $f^*=30$~Hz is the lowest high-frequency cutoff used in the search template bank as it provides the maximum angle between the line of sight and the cusp/kink on the loop. The parameter space of model $M$, $(G\mu,p)$, is scanned and excluded at a \red{95\%} level when  ${\cal{R}}^{(M)}_q$ exceeds \red{$2.996/T_{\rm{obs}}$} which is the rate expected from a random Poisson process over an observation time $T_{\rm{obs}}$. The resulting constraints are shown in Fig.~\ref{fig:contours} and will be discussed in Sec~\ref{sec:conclusion}.
\begin{figure*}
  \center
  \epsfig{width=8cm, file=./Figures/burst_cusprate.eps} \epsfig{width=8cm, file=./Figures/burst_kinkrate.eps}\\
  \epsfig{width=8cm, file=./Figures/burst_cuspeff.eps} \epsfig{width=8cm, file=./Figures/burst_kinkeff.eps}
  \caption{In the upper plots, the red points show the measured cumulative cusp (left-hand plot) and kink (right-hand plot) GW burst rate (using $T_{\rm{obs}}$ as normalization)  as a function of the likelihood ratio $\Lambda$. The black line shows the expected background of the search with the $\pm 1\sigma$ statistical error represented by the hatched area. In both cases, the highest-ranked event ($\Lambda_h \simeq 232$ and $\Lambda_h \simeq 611$) is consistent with the background. The lower plots show the sensitivity of the search as a function of the cusp/kink signal amplitude. This is measured by the fraction of simulated cusp/kink events recovered with $\Lambda > \Lambda_h$. The sensitivity to cusp signals is also measured for a false-alarm rate (FAR) of $1.85 \times 10^{-6}$~Hz to be compared with the sensitivity of the previous LIGO-Virgo burst search~\cite{Aasi:2013vna} (dashed lines).}
  \label{fig:burst}
\end{figure*}


\subsection{Stochastic gravitational-wave background}\label{sec:data:stochastic}
\textcolor{red}{Cosmic string networks also generate a stochastic background of GWs, which is measured
using the energy density
\be
\Omega_{\rm{GW}}(f) = \frac{f}{\rho_c}\frac{d\rho_{\rm{GW}}}{df},
\ee
where $d\rho_{\rm{GW}}$ is the energy density of GWs in the frequency range $f$ to 
$f + df$ and $\rho_{c}$ is the critical energy density of the Universe. 
Following the method outlined in \cite{Olmez:2010bi}, the GW energy density 
is given by:
%
\begin{align}
\Omega^{(M)}_{\rm{GW}}(f;G\mu,p) =& \frac{4\pi^2}{3H_0^2}f^3\int_0^{h^{*}}dh\ h^2
\nonumber \\
& \times \int_0^{+\infty}dz \frac{d^2R^{(M)}}{dzdh}(h,z,f;G\mu,p),
\label{eq:spec}
\end{align}
%
%\be
%\Omega^M_{GW}(f) = \frac{4\pi^2}{3H_0^2}f^3 \int_{z_\mathrm{min}}^{z_\mathrm{max}}dz% \int_{h_\mathrm{min}(z)}^{h^{*}}dh\ h^2\frac{d^2R^M}{dzdh}(h,z,f),
%\label{eq:spec_zh}
%\ee
%
where the spectrum is computed for a specific 
choice of free parameters $G\mu$ and $p$, and the maximum strain amplitude $h^{*}$ is defined below. 
This equation gives the contribution to the stochastic background from the 
superposition of unresolved signals from cosmic string cusps and kinks, and we shall determine the total GW energy density due to cosmic strings is by summing the two. Note that this calculation {\it underestimates} the stochastic background since it only includes the high-frequency contribution from kinks and cusps. The low-frequency contribution from the smooth part of loops may be important, and has been discussed in \cite{Blanco-Pillado:2017rnf,Blanco-Pillado:2017oxo,Ringeval:2017eww,Binetruy:2012ze}. Neglecting this contribution, conservative constraints will be derived.}

To compute the integrals in 
Eq.~\ref{eq:spec} we adopt the numerical method described in 
Appx.~\ref{appx:tech}.
As observed in~\cite{Damour:2000wa}, the 
integration over the strain amplitude is performed up to $h^{*}$ to exclude the individually resolvable 
powerful and rare bursts. The maximum strain amplitude $h^{*}$ determined by solving the equation
%as those will not be included in the searches for the stochastic background.
%Consequently, the $h$ integration is performed up 
%to a maximum strain amplitude $h^{*}$ determined by solving the equation
\be
\int_{h^{*}}^{+\infty}dh\int_{0}^{+\infty}dz \frac{d^2R^{(M)}}{dzdh}(h,z,f) = f.
\label{eq:hstar}
\ee
This encodes the fact that when the burst rate is larger than $f$, individual bursts are not resolved.

The total energy density in gravitational waves produced by cosmic strings will be composed of overlapping signals ($h < h^{*}$) and non-overlapping signals, namely bursts ($h > h^{*}$). The LIGO-Virgo stochastic search pipeline will detect both types of signals. This has been demonstrated for a stochastic background produced by binary neutron stars, whose signals overlap, and binary black holes, whose signals will arrive in a non-overlapping fashion~\cite{Meacher:2015iua,Abbott:2017xzg}. In this present cosmic string study this effect is negligible: the predicted GW energy density, $\Omega^{(M)}_{\rm{GW}}$,  does not grow significantly (and Fig.~\ref{fig:spectrum}, top, does not change noticeably) when $h^* \rightarrow +\infty$.

Fig.~\ref{fig:spectrum} (top) shows the spectra for the three models under 
consideration,
adding both the cusp and the kink contributions and assuming $G\mu=10^{-8}$. 
Model 2 spectrum is about 10 times weaker than the spectrum of model 1 
over most of the frequency range. As shown in Fig.~\ref{fig:spectrum_03} (top),
the spectra are dominated by the contribution of loops in the radiation era 
over most of the frequency range,
including the frequencies accessible to LIGO and Virgo detectors (10-1000 Hz).
The difference in normalizations
of the loop distributions in the radiation era in the two models, 
discussed in Sec.~\ref{sec:models}, is therefore
the cause for the difference in spectral amplitudes. Note also that at
low frequencies ($\sim 10^{-9}$ Hz), at which pulsar timing observations 
are made, the matter era loops contribute the most.

Fig.~\ref{fig:spectrum} (top) also shows that the spectrum for model 3 has a significantly higher amplitude than those of models 1 and 2. Fig.~\ref{fig:spectrum_03} shows that this spectrum is dominated by the contribution of small loops which, as discussed in Sec.~\ref{sec:models}, are much more numerous in model 3.

Fig.~\ref{fig:spectrum} (bottom) shows the maximum value for the 
strain amplitude to consider in the integration, $h^*$ as a 
function of the frequency. At LIGO-Virgo frequencies (10-1000 Hz) the 
spectrum originates from GWs with strain amplitudes below $\sim 10^{-28}$.

\begin{figure}
  \center
  \epsfig{width=7.7cm, file=./Figures/spectrum.eps}
  \epsfig{width=7.7cm, file=./Figures/hstar.eps}
  \caption{Top: GW energy density, $\Omega^{(M)}_{\rm{GW}}(f)$, from cusps and kinks 
predicted by the three loop distribution models. The string tension $G\mu$ has 
been fixed to $10^{-8}$. Bottom: maximum strain amplitude $h^{*}$ used 
for the integration in Eq.\ref{eq:spec}.}
  \label{fig:spectrum}
\end{figure}
%
\begin{figure}
  \center
  \epsfig{width=7.7cm, file=./Figures/spectrum_0.eps}
  \epsfig{width=7.7cm, file=./Figures/spectrum_3.eps}
  \caption{Top: GW energy density, $\Omega^{(M)}_{\rm{GW}}(f)$, from cusps for model 1. We have separated the contributions 
from loops in the radiation ($z>3366$) and matter ($z<3366$) eras. 
Additionally, for loops in the matter era, we have separated the effect 
of loops produced in the matter era from the ones produced in the 
radiation era (Eq.~\ref{dist-rad}, Eq.~\ref{dist-1} and Eq.~\ref{dist-2}). 
Bottom: GW energy density, $\Omega^{(M)}_{\rm{GW}}(f)$, from cusps for model 3. The effect of the three loop 
size regimes is shown (Eq.~\ref{eq:mod3_1}, Eq.~\ref{eq:mod3_2} and 
Eq.~\ref{eq:mod3_3}) for the matter and radiation eras.}
  \label{fig:spectrum_03}
\end{figure}

The energy density spectra predicted by the models can be compared with several
observational results. First, searches for the stochastic GW 
background using LIGO and Virgo detectors have been performed, using
the initial generation detectors (science run S6, 2009-2010)~\cite{Aasi:2014zwg} and the first 
observation run (O1, 2015-2016) of the advanced
detectors~\cite{TheLIGOScientific:2016dpb}. Both searches reported frequency-dependent
upper limits on the energy density in GWs. To translate these
upper limits into constraints on cosmic string parameters, we define the 
following likelihood function:
%
\begin{equation}
\ln L(G\mu,p)\propto \sum_i \frac{-\left( Y(f_i) - \Omega^{(M)}_{\rm{GW}}(f_i; G\mu,p)
\right)^2}{\sigma^2(f_i)} ,                                                
\label{stochlik}
\end{equation}                                                                       %                                                                     
where $Y(f_i)$ and $\sigma(f_i)$ are the measurement and the associated 
uncertainty of the GW energy density in the frequency bin $f_i$, 
and $\Omega_{\rm{GW}}^{(M)}(f_i;G\mu,p)$ is the energy density computed by a cosmic 
string model at the same frequency bin $f_i$ and for some set of model 
parameters $G\mu$ and $p$. We evaluate the likelihood function across 
the parameter space $(G\mu,p)$ and compute the \red{95\%} confidence contours for 
the initial LIGO-Virgo (S6, $41.5<f<169$~Hz)~\cite{Aasi:2014zwg} and for the most 
recent Advanced LIGO (O1, $20<f<86$~Hz)~\cite{TheLIGOScientific:2016dpb} stochastic 
background measurements (assuming Bayesian formalism and 
flat priors in the log parameter space). 
Since a stochastic background of GWs has not been detected yet, these 
contours define the excluded regions of the parameter space. We also compute 
the projected design sensitivity for the Advanced LIGO and Advanced Virgo 
detectors, using Eq.~\ref{stochlik} with $Y(f_i) = 0$ and with the 
projected $\sigma(f_i)$ for the detector network \cite{TheLIGOScientific:2016wyq}.

Another limit can be computed based on the Pulsar Timing Array (PTA) 
measurements of the pulse arrival times of millisecond pulsars
~\cite{Lasky:2015lej}. This measurement produces a limit on the energy
density at nanohertz frequencies --- specifically, at 95\% confidence
$\Omega_{\rm{GW}}^{\rm{PTA}}(f=2.8\times 10^{-9}\mathrm{~Hz})<2.3\times 10^{-10}$. We directly
compare the spectra predicted by our models (at $2.8\times 10^{-9}\mathrm{~Hz}$)
to this constraint.

Finally, indirect limits on the total (integrated over frequency) energy 
density in GWs can be placed based on the Big-Bang Nucleosynthesis
(BBN) and Cosmic Microwave Background (CMB) observations. The BBN model and 
observations of the abundances of the lightest nuclei can be used to
constrain the effective number of relativistic degrees of freedom at the time
of the BBN, $N_{\mathrm{eff}}$. Under the assumption that only photons and 
standard light neutrinos contribute to the radiation energy density, 
$N_{\mathrm{eff}}$ is equal to the effective number of neutrinos, corrected 
for the residual heating of the neutrino fluid due to electron-positron 
annihilation: $N_{\mathrm{eff}} \simeq 3.046$~\cite{Mangano:2005cc}. 
Any deviation from this value can be attributed to extra relativistic radiation,
including potentially GWs due to cosmic string kinks and cusps
generated prior to BBN. We therefore use the 95\% confidence upper limit
$N_{\mathrm{eff}} - 3.046 < 1.4$, obtained by comparing the BBN model and the 
abundances of deuterium and $^4{\rm He}$ ~\cite{Cyburt:2004yc}, which translates into
the following limit on the total energy density in GWs:
%
\begin{equation}
\Omega^{\rm{BBN}}_{\rm{GW}} (G\mu,p)  =  \int_{10^{-10}{\rm ~Hz}}^{10^{10} {\rm ~Hz}}df
\Omega_{\rm{GW}}^{(M)}(f;G\mu,p) < 1.75 \times 10^{-5},
\label{om_bbn}
\end{equation}
%
where the lower bound on the integrated frequency region is determined by 
the size of the horizon at the time of BBN~\cite{Binetruy:2012ze}.
In this calculation we only consider kinks and cusps generated before 
BBN, which implies limiting the redshift integral in Eq.~\ref{eq:spec} to
$z>5.5\times 10^{9}$.

Similarly, presence of GWs at the time of photon decoupling
could alter the observed CMB and Baryon Acoustic Oscillation spectra. We apply
a similar procedure as in the BBN case, integrating over redshifts before
the photon decoupling ($z>1089$) and over all frequencies above $10^{-15}$ Hz
(horizon size at the time of decoupling) to compute
the total energy density of GWs at the time of decoupling.
We then compare this quantity to the posterior 
distribution obtained in~\cite{Pagano:2015hma} to compute the \red{95\%}
confidence contours:
%
\begin{equation}
\Omega^{\rm{CMB}}_{\rm{GW}} (G\mu,p)  =  \int_{10^{-15}{\rm ~Hz}}^{10^{10} {\rm ~Hz}}df
\Omega_{\rm{GW}}^{(M)}(f;G\mu,p) < 3.7 \times 10^{-6},
\label{om_cmb}
\end{equation}
%



%Nucleosynthesis (BBN) and the cosmic microwave background (CMB) monopole 
%can be used to measure $N_{\mathrm{eff}}$ so that they provide indirect upper 
%bounds on $h_0^2\Omega_{GW}$. These measurements constrain the total 
%relativistic energy density of the universe at photon decoupling 
%($z_\mathrm{CMB}=1089$) and at the time of nucleosynthesis 
%($z_\mathrm{BBN}=5.5 \times 10^9$) for the CMB and BBN respectively. 
%As a result, when integrating the GW rate in Eq.~\ref{eq:spec_zh}, 
%one must consider $z_\mathrm{min}=z_\mathrm{CMB},z_\mathrm{BBN}$ for the 
%redshift integral. Moreover the total GW energy density, $\Omega_{GW}$, 
%is obtained by integrating the spectrum over all the relevant frequencies:
%\ba
%\Omega^{CMB}_{GW} &=& \int_{10^{-16}}^{+\infty}df\Omega_{GW}(f) \\
%\Omega^{BBN}_{GW} &=& \int_{10^{-10}}^{+\infty}df\Omega_{GW}(f).
%\ea

For reference, Fig.~\ref{fig:spectrum_ccncmb} shows the energy density spectra
for models 1 and 3 using $G\mu=10^{-8}$. As expected, 
the contribution from the matter era loops is suppressed at the time of the BBN
or of photon decoupling, resulting in the suppression of the spectra at low 
frequencies. To have negligible systematic errors associated to the numerical integration, we compute Eq.~\ref{om_bbn} and Eq.~\ref{om_cmb} using 200 and 250 logarithmically-spaced frequency bins respectively.
%
\begin{figure}
  \center
  \epsfig{width=8cm, file=./Figures/spectrum_bbncmb.eps}
  \caption{GW energy density, $\Omega^{(M)}_{\rm{GW}}(f)$, from cusps for models 1 and 3. The spectra have 
been computed at the time of photon decoupling ($z_\mathrm{CMB}=1100$) and at 
the time of nucleosynthesis ($z_\mathrm{BBN}=5.5 \times 10^9$).}
  \label{fig:spectrum_ccncmb}
\end{figure}

Fig.~\ref{fig:contours} shows the excluded regions in the parameter spaces of
the three models considered here, based on the stochastic observational constraints
discussed above.
%
\begin{figure*}[!tp]
  \centering
  \begin{subfigure}[t]{0.48\textwidth}
    \includegraphics[width=\textwidth]{./Stochastic/Output/Figures/Siemens3.eps}
  \end{subfigure}
  \begin{subfigure}[t]{0.48\textwidth}
    \includegraphics[width=\textwidth]{./Stochastic/Output/Figures/Olum3.eps}
  \end{subfigure}
  \begin{subfigure}[t]{0.48\textwidth}
    \includegraphics[width=\textwidth,valign=c]{./Stochastic/Output/Figures/Ringeval3.eps}
  \end{subfigure}
  \begin{subfigure}[t]{0.48\textwidth}
    \includegraphics[width=0.6\textwidth,valign=c]{./Stochastic/Output/Figures/Legend3.eps}
  \end{subfigure}
  \caption{\red{95\%} confidence exclusion regions are shown for three loop 
    distribution models: $M=1$ (top-left), 
    $M=2$ (top-right), and 
    $M=3$ (bottom-left). Shaded regions are excluded by the 
    latest (O1) Advanced LIGO stochastic \cite{TheLIGOScientific:2016dpb} and burst 
    (presented here) measurements. We also show the bounds from the previous 
    LIGO-Virgo stochastic 
    measurement (S6) \cite{Aasi:2014zwg}, from the indirect BBN and CMB bounds 
    \cite{Cyburt:2004yc,Pagano:2015hma}, and from the PTA measurement (Pulsar) \cite{Lasky:2015lej}. 
    Also shown is the projected design sensitivity of 
    the Advanced LIGO and Advanced Virgo experiments (Design, Stochastic) 
    \cite{TheLIGOScientific:2016wyq}. The excluded regions are below the 
    respective curves.}
  \label{fig:contours}
  
\end{figure*}

          


